Hot Gas Lines in T Tauri Stars

For Classical T Tauri Stars (CTTSs), the resonance lines of N V, Si IV, and C IV, as well as the He II 1640 A line, act as diagnostics of the accretion process. Here we assemble a large high-resolution dataset of these lines in CTTSs and Weak T Tauri Stars (WTTSs). We present data for 35 stars: one Herbig Ae star, 28 CTTSs, and 6 WTTSs. We decompose the C IV and He II lines into broad and narrow Gaussian components (BC & NC). The most common (50 %) C IV line morphology in CTTSs is that of a low-velocity NC together with a redshifted BC. The velocity centroids of the BCs and NCs are such that V_BC > 4 * V_NC, consistent with the predictions of the accretion shock model, in at most 12 out of 22 CTTSs. We do not find evidence of the post-shock becoming buried in the stellar photosphere due to the pressure of the accretion flow. The He II CTTSs lines are generally symmetric and narrow, less redshifted than the CTTSs C IV lines, by ~10 km/sec. The flux in the BC of the He II line is small compared to that of the C IV line, consistent with models of the pre-shock column emission. The observations are consistent with the presence of multiple accretion columns with different densities or with accretion models that predict a slow-moving, low-density region in the periphery of the accretion column. For HN Tau A and RW Aur A, most of the C IV line is blueshifted suggesting that the C IV emission is produced by shocks within outflow jets. In our sample, the Herbig Ae star DX Cha is the only object for which we find a P-Cygni profile in the C IV line, which argues for the presence of a hot (10^5 K) wind. For the overall sample, the Si IV and N V line luminosities are correlated with the C IV line luminosities, although the relationship between Si IV and C IV shows large scatter about a linear relationship and suggests that TW Hya, V4046 Sgr, AA Tau, DF Tau, GM Aur, and V1190 Sco are silicon-poor.

==> TableAncil.tex <==
%\documentclass[12pt,preprint]{/Users/ardila/aastex52/aastex}
%\begin{document}
\begin{deluxetable}{lccccccccccccccccc}
\rotate
\tablecolumns{18}
\tabletypesize{\tiny}
\tablewidth{0pt}
\tablecaption{Stars used in this paper\label{TableAncil}}
\tablehead{\colhead{Name (a)} & \colhead{Alternate name} & \colhead{Region} & \colhead{Type?} & \colhead{SpT} & \colhead{Ref. SpT} & \colhead{Radial Velocity (\kms)} & \colhead{Ref. Rad. Vel.} & \colhead{Inclination (b)} & \colhead{Ref. Inclination} & \colhead{Av} & \colhead{Ref. Av} & \colhead{Binary? (c)} & \colhead{Ref. Binary} & \colhead{M (msun)} & \colhead{Ref. M} & \colhead{Radius (d)} & \colhead{Ref. Radius}} 
\startdata

AA Tau & HBC 63 & Taurus-Auriga & CTTS & K7 & Donati et al. (2010) & 16.5 & 
Bouvier et al. (1999) & 70$\pm$10 & Donati et al. (2010) & 0.8 & 
Bouvier et al. (1993) & S & Najita et al. (2007) & 0.7 & Siess et al. (2000) & 
2 & Siess et al. (2000) \\ 
AK Sco & HBC 271  & Upper-Scorpius & CTTS & F5 & Andersen et al. (1989) & 
-1.15 & Andersen et (1989) & 63 & Andersen et (1989) & 0.5 & 
Alencar et al. (2003) & 2 (SB) & Alencar et al. (2003) & 1.35 x 2 & 
Alencar et al. (2003) & 1.59 x 2 & Alencar et al. (2003) \\ 
BP Tau & HBC 32 & Taurus-Auriga & CTTS & K7 & Johns-Krull et al. (1999) & 
15.8 & Hartmann et al. (1986) & 20$\pm$20 & Simon et al. (2000) & 0.5 & 
Gullbring et al. (1998) & S & Leinert et al. (1993) & 0.70 $\pm$ 0.15  & 
Siess et al. (2000) & 1.95$\pm$0.26 & Johns-Krull et al. (1999) \\ 
CS Cha & HBC 569 & Chamaeleon I & CTTS & K6 & Luhman et al. (2004) & 15.0 & 
Reipurth et al. ((1995)) & TBD & TBD & 0.3 & Furlan et al. (2009) & 2 (SB) & 
Guenther et al. (2007) & TBD & TBD & 2.07 & Derived from Luhman (2007) \\ 
CV Cha & HBC 247 & Chamaeleon I & CTTS & G8 & Guenther et al. (2007) & 16.1 & 
Guenther et al. (2007) & 35$\pm$10 & Hussain et al. (2002) & 1.5 & 
Furlan et al. (2009) & S & Melo et al. (2003) & 2$\pm$0.15 & 
Hussain et al. (2002) & 2.5$\pm$0.4 & Hussain et al. (2002) \\ 
CY Tau & HBC 28 & Taurus-Auriga & CTTS & M1 & Hartmann et al. (1998) & 19.1 & 
Hartmann et al. (1986) & 47$\pm$8 & Simon et al. (2000) & 1.7 & 
Furlan et al. (2009) & S & Najita et al. (2007) & 0.58 & 
Johns-Krull \& Gafford (2002) & 1.4 & Johns-Krull \& Gafford (2002) \\ 
DE Tau & HBC 33 & Taurus-Auriga & CTTS & M0 & Furlan et al.(2009) & 14.9 & 
Hartmann et al. (1986) & 57 & Appenzeller et al. (2005) & 1.2 & 
Furlan et al. (2009) & S & Najita et al. (2007) & 0.23 & 
Johns-Krull \& Gafford (2002) & 6.34 & Johns-Krull \& Gafford (2002) \\ 
DF Tau & HBC 36  & Taurus-Auriga & CTTS & M2 & Herczeg et al. (2008) & 11.0 & 
Edwards et al. (1987) & 50 & Appenzeller et al. (2005) & 0.6 & 
Herczeg et al. (2008) & "2 (0.09"")" & Ghez et al. (1993) & 0.66 & 
Herczeg et al. (2008) & 3.2 & Herczeg et al. (2008) \\ 
DK Tau & HBC 45 & Taurus-Auriga & CTTS & K7 & Furlan et al.(2009) & 15.3 & 
Hartmann et al. (1986) & 44 & Appenzeller et al. (2005) & 1.3 & 
Furlan et al.(2009) & "2 (2.304"")" & 
Correia et al. (2006) (Binary star DB - Lowell Obs) & 0.52 & 
Johns-Krull \& Gafford (2002) & 1.53 & Johns-Krull \& Gafford (2002) \\ 
DM Tau & HBC 62 & Taurus-Auriga & CTTS & M1.5 & Espaillat et al. (2010) & 
16.9 & Hartmann et al. (1986) & 45$\pm$5 & Simon et al. (2000) & 0.6 & 
Ingleby et al. (2009) & S & Najita et al. (2007) & 0.53 & 
Cohen \& Kuhi (1979)  & 1.25 & Salyk et?al. (2009) \\        
DN Tau & HBC 65 & Taurus-Auriga & CTTS & M0 & Furlan et al.(2009) & 16.1 & 
Hartmann et al. (1986) & 30 & Appenzeller et al. (2005) & 0.6 & 
Furlan et al.(2009) & S & Najita et al. (2007) & 0.47 & 
Johns-Krull \& Gafford (2002) & 2.39 & Johns-Krull \& Gafford (2002) \\ 
DR Tau & HBC 74 & Taurus-Auriga & CTTS & K7 & Petrov et al. (2011) & 27.6 & 
Alencar \& Basri (2000). & 20$\pm$4 & Petrov et al. (2011) & 1.6 & 
Gullbring et al. (1998) & S & Leinert et al. (1993) & 0.38 & 
Johns-Krull \& Gafford (2002) & 2.7 & Johns-Krull \& Gafford (2002) \\ 
DS Tau & HBC 75 & Taurus-Auriga & CTTS & K5 & Muzerolle et al. (1998) & 16.3 & 
Hartmann et al. (1986)  & $\sim$90 & 
Derived from Kundurthy et al. (2006); Glebocki et al. (2005) (b) & 1.1 & 
Furlan et al.(2009) & S & Najita et al. (2007) & 1.04 & White \& Ghez (2001) & 
1.42 & Derived from Kundurthy et al. (2006) \\ 
DX Cha & HD 104237 & eps Chamaeleontis & CTTS & A7.5 & Grady et al (2004) & 
13 & Kharchenko+; (2007); & 18 & Grady et al (2004) & 0.51 & 
Sartori et al. (2003) & 2 (SB) & Bohm et al. (2004) & TBD & TBD & 7.05 & 
Derived from Ammons et al. (2006); Sartori et al. (2003) \\ 
EG Cha & RECX 1 & eta Chamaeleontis & WTTS & K4 & Mamajek et al. (1999) & 18 & 
Malaroda+; (2006); & N/A & N/A & 0 & Ingleby et al. (2011) & 
"M (AB 0.18""; AB-C: 8.6"")" & Kohler \& Petr-Gotzens ((2002)) & 0.9 & 
Ingleby et al. (2011) & 1.8 & Ingleby et al. (2011) \\       
EP Cha & RECX 11 & eta Chamaeleontis & CTTS & K4 & Mamajek et al. (1999) & 18 & 
Assumed as EG Cha & Not found & Not found & 0 & 
Ingleby et al. (2011) & S & Brandeker et al. (2006) & 1 & 
Ingleby et al. (2011) & 1.4 & Ingleby et al. (2011) \\ 
ET Cha & RECX 15 & eta Chamaeleontis & CTTS & M2 & Lawson et al. (2002) & 
15.9 & Andersen et al. (1975) & $\sim$90 & 
Derived from AAVSO; Glebocki et al. (2005) (b) & 0 & Ingleby et al. (2011) & 
S & Kohler \& Petr-Gotzens ((2002)) & 0.35 & Lawson et al. (2002) & 1 & 
Assumed \\ 
GM Aur & HBC 77 & Taurus-Auriga & CTTS & K5.5 & Espaillat et al. (2010) & 
14.8 & Simon et al. (2000) & 54$\pm$5 & Simon et al. (2000) & 1.2 & 
Espaillat et al. (2010) & S & Najita et al. (2007) & 0.56 & 
Johns-Krull \& Gafford (2002) & 1.42 & Johns-Krull \& Gafford (2002) \\ 
HN Tau & HBC 60 & Taurus-Auriga & CTTS & K5 & Furlan et al.(2009) & 4.6 & 
Nguyen et al. (2012) & Not found & Not found & 1.5 & Furlan et al.(2009) & 
"2 (3.109"")" & Correia et al. (2006) (Binary star DB - Lowell Obs) & 
1.0$\pm$0.1 & White \& Ghez (2001) & 1.48 & Derived from Palla et al. (2002) \\ 
IP Tau & HBC 385 & Taurus-Auriga & CTTS & M0 & Furlan et al.(2009) & 14.8 & 
Hartmann et al. (1987) & 29.4 &                              
Derived from Kundurthy et al. (2006); Glebocki et al. (2005) (b) & 0.5 & 
Furlan et al.(2009) & S & Najita et al. (2007) & 0.52 & 
Johns-Krull \& Gafford (2002) & 1.44 & Johns-Krull \& Gafford (2002) \\ 
MP Mus & PDS 66 & Isolated? & CTTS & K1 & Torres et al. (2006) & 11.6 & 
Torres et al. (2006) & 32 & Curran et al. (2011) & 0.17 & 
Mamajek et al. (2002) & Not found & Not found & 1.2 & Curran et al. (2011) & 
1.3 & Curran et al. (2011) \\ 
RU Lup & HBC 251  & Lupus I & CTTS & K7 & Herczeg et al. (2005) & -0.9 & 
Melo (2003) & 24 & Herczeg et al. (2005) & 0.1 & Herczeg et al. (2008) & S & 
Lamzin et al. ((1995)) & 1.0 & Herczeg et al. (2008) & 1.3 & 
Herczeg et al. (2008) \\ 
RW Aur & HBC 80  & Taurus-Auriga & CTTS & K4 & Johns-Krull et al. (1999) & 
14.0 & Hartmann et al. (1986) & 37 & Appenzeller et al. (2005) & 1.14 & 
Johns-Krull et al. (1999) & "M (A-BC 1.41""; BC: 0.12"")" & 
Correia et al. (2006) (Binary star DB - Lowell Obs) & 0.8 & 
Johns-Krull \& Gafford (2002) & 1.46 & Johns-Krull \& Gafford (2002) \\ 
SU Aur & HBC 79 & Taurus-Auriga & CTTS & G1 & Furlan et al.(2009) & 9.7 & 
Hartmann et al. (1986) & 52$\pm$10 & Akeson et al. (2005) & 0.9 & 
Furlan et al.(2009) & S & Nguyen et al. (2012) & 2.25 & Cohen et al. (1989) & 
3.6 & Johns \& Basri (1995) \\ 
T Tau N & HBC 35 & Taurus-Auriga & CTTS & K1 & Walter et al. (2003) & 19 & 
Hartmann et al. (1986) & 19 & Herbst et al. (1997) & 1.2 & 
Walter et al. (2003) & "2 (0.7"")" & Dyck et al. 1982 & 2.11$\pm$0.18 & 
White \& Ghez (2001) & 3.4 & Herbst et al. (1997) \\ 
TW Hya & HBC 568 & TW Hydrae Association & CTTS & K6 & Torres et al. (2006) & 
13.5 & Sterzik et al. (1999); measured by Herczeg et al. (2002); & 18$\pm$10 & 
Herczeg et al. (2002) & 0.0 & Herczeg et al. (2004) & S & 
Curran et al. (2011) & 0.77 & Herczeg et al. (2008) & 0.83 & 
Herczeg et al. (2008) \\ 
TWA 3A & Hen 3-600A & TW Hydrae Association & CTTS & M4 & 
Torres et al. (2006) & 10.4 & de la Reza et al. (1989) & 0 & 
Curran et al. (2011) & 0.7 & Curran et al. (2011) & "2 (1.4"")" & 
Correia et al. (2006) (Binary star DB - Lowell Obs) & 0.2 & 
Curran et al. (2011) & 0.9 & Curran et al. (2011) \\ 
TWA 7 & 2MASS J1042-3340  & TW Hydrae Association & WTTS & M2 & 
Torres et al. (2006) & 10.6 & Kharchenko+; (2007); & N/A & N/A & 0 & 
Ingleby et al. (2009) & S & Lowrance et al. (2005) & TBD & TBD & TBD & TBD \\ 
UX Tau A & HBC 43 & Taurus-Auriga & CTTS & K2 & Herbig (1977) & HOPR & HOPR & 
49 & Andrews et al. (2011) & 1.8 & Espaillat et al. (2010) & S & 
Najita et al. (2007) & 1.5 & Espaillat et al. (2010) & 1.8 & 
Espaillat et al. (2010) \\ 
V1068 Tau & LkCa 4; HBC 370 & Taurus-Auriga & WTTS & K7 &    
Herbig \& Bell (1988) & 16.9 & Hartmann et al. (1987) & N/A & N/A & 0.69 & 
Bertout et al. (2007) & S & Najita et al. (2007) & 0.77 & 
Bertout et al. (2007) & 1.87 & Derived from Palla et al. (2002) \\ 
V1079 Tau  & LkCa 15; HBC 419  & Taurus-Auriga & CTTS & K3 & 
Espaillat et al. (2010) & 17.0 & Hartmann et al. (1987) & 42$\pm$5 & 
Simon et al. (2000) & 1.7 & Espaillat et al. (2010) & S & 
Najita et al. (2007) & 1.3 & Espaillat et al. (2010) & 1.6 & 
Espaillat et al. (2010) \\ 
V1190 Sco & HBC 617 & Upper Scorpius & CTTS & K0 & Hughes et al.(1994) & 5.0 & 
Graham et al. (1988) & $<$5 & Comeron \& Fernandez (2010) & 0.32 & 
Sartori et al. (2003) & Not found & Not found & 0.9 & 
Comeron \& Fernandez (2010) & 1.99 & Derived from Evans et al. (2009) \\ 
V2129 Oph & HBC 264 & Rho Ophiuchus & CTTS & K5 & Wilking et al. (2005) & 
-7.1 & Torres et al. (2006) & 45 & Curran et al. (2011) & 0.3 & 
Curran et al. (2011) & S & Curran et al. (2011) & 1.35 & Curran et al. (2011) & 
2.4 & Curran et al. (2011) \\ 
V396 Aur & LkCa 19; HD 282630 & Taurus-Auriga & WTTS & K0 & 
Herbig \& Bell (1988) & 14.3 & Hartmann et al. (1987) & N/A & N/A & 0 & 
Walter et al. (1988) & S & Najita et al. (2007) & 1.3 & 
Massarotti et al. (2005) & 1.58 & Derived from Palla et al. (2002) \\ 
V397 Aur & HBC 427 & Taurus-Auriga & WTTS & K7; M2 & Steffen et al. (2001) & 
15.0 & Walter et al. (1988) & N/A & N/A & 0.15 & Steffen et al. (2001) & 
"2 (0.0328"")" & Steffen et al. (2001) & 1.45$\pm$0.19; 0.81$\pm$0.09 & 
Steffen et al. (2001) & 1.83 & Derived from Palla et al. (2002) \\ 
V4046 Sgr & HBC 662 & Isolated? & CTTS & K5 & Curran et al. (2011) & -7.0 & 
Malaroda+; (2006); & 35 & Curran et al. (2011) & 0 & Curran et al. (2011) & 2 & 
Curran et al. (2011) & 0.86 & Curran et al. (2011) & 1.16 & 
Curran et al. (2011) \\ 
V410 Tau & HBC 29 & Taurus-Auriga & WTTS & M6 & Furlan et al.(2009) & 17.8 & 
Hartmann et al. (1986) & N/A & N/A & 0.03 & Bertout et al. (2007) & 
"M (AB-C: 0.290; AB: 0.07"")" & Binary star DB - Lowell Obs & 1.45 & 
Bertout et al. (2007) & 2.18 & Derived from Palla et al. (2002) \\ 

\enddata
\tablecomments{
(a) In this paper we refer to the stars with their variable star name, if it exists. The exceptions are the TWA members which do not have variable star names.\\
(b) When inclination is listed as "Derived from" we have derived ourselves from $v * \sin I$, period, and radius\\
(c) S: Single; 2: Double, either spectroscopic binary (SB) or components with the separation given; M: Multiple
(d)  When radius is listed as "Derived from" we have derived ourselves from the luminosity and effective temperature.}

\end{deluxetable}
%\end{document}


